ML-FEED: Machine Learning Framework for Efficient Exploit Detection

Machine learning (ML)-based methods have recently become attractive for detecting security vulnerability exploits. Unfortunately, state-of-the-art ML models like long short-term memories (LSTMs) and transformers incur significant computation overheads. This overhead makes it infeasible to deploy them in real-time environments. We propose a novel ML-based exploit detection model, ML-FEED, that enables highly efficient inference without sacrificing performance. We develop a novel automated technique to extract vulnerability patterns from the Common Weakness Enumeration (CWE) and Common Vulnerabilities and Exposures (CVE) databases. This feature enables ML-FEED to be aware of the latest cyber weaknesses. Second, it is not based on the traditional approach of classifying sequences of application programming interface (API) calls into exploit categories. Such traditional methods that process entire sequences incur huge computational overheads. Instead, ML-FEED operates at a finer granularity and predicts the exploits triggered by every API call of the program trace. Then, it uses a state table to update the states of these potential exploits and track the progress of potential exploit chains. ML-FEED also employs a feature engineering approach that uses natural language processing-based word embeddings, frequency vectors, and one-hot encoding to detect semantically-similar instruction calls. Then, it updates the states of the predicted exploit categories and triggers an alarm when a vulnerability fingerprint executes. Our experiments show that ML-FEED is 72.9x and 75,828.9x faster than state-of-the-art lightweight LSTM and transformer models, respectively. We trained and tested ML-FEED on 79 real-world exploit categories. It predicts categories of exploit in real-time with 98.2% precision, 97.4% recall, and 97.8% F1 score. These results also outperform the LSTM and transformer baselines.

==> background_old.tex <==
\section{Background}
\label{sec:background}
This section discusses background material for program representations and machine learning models.

\begin{comment}

\subsection{Call Graph}
A call graph is a control-flow graph representing the calling relationships between functions in a 
program. Fig.~\ref{fig:callgraph} shows an example of a call graph where each node represents a function, and each edge represents the calling relationship between the functions. For example, if a function $f_1$ calls $f_2$ during the program flow, the calling relationship is represented by a directed edge ($f_1$,$f_2$). 
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.55]{images/callgraph.pdf}
    \caption{Example of a call graph.}
    \label{fig:callgraph}
\end{figure}

\end{comment}

\subsection{System Dependence Graph}
In this paper, we use a \textit{System Dependence Graph} (\texttt{SDG})~\cite{walkinshaw2003java} as the inter-procedural graph representation of programs to extract the vulnerable API sequences for training our model. An SDG $\mathcal{G} = (V, E^{c}, E^{d})$ is a three-tuple, where $V$ represents program statements, $E^{c}$ encodes control dependency edges, and $E^{d}$ denotes data dependency 
edges.  For nodes $X$ and $Y$ in an SDG, $Y$ is control-dependent on $X$ if,
during execution, $X$ can directly affect whether $Y$ is executed.
Also, $X$ is data-dependent on $Y$ if $Y$ is an assignment and  
 $X$ can access the value assigned in $Y$. 
Since these data and control dependencies are computed for individual program procedures (or functions), 
they do not account for inter-procedural control and data relationships. As a result, they cannot determine 
the transitive dependencies by default. Therefore, we augment the SDG with information on inter-procedural 
relationships. SDG edges also represent the direct dependence between the call site and the 
called procedure, which allows us to determine the transitive dependencies due to a call. 

\begin{figure}[h]
    \centering
    \vspace{-0.2cm}
    \includegraphics[scale=0.7]{images/sdg.pdf}
    \caption{Example of an SDG for call graph nodes 1 and 2. Here, an SDG node represents a 
statement and an edge represents the control or data dependency between program statements.}
    \label{fig:sdg}
\end{figure}

An SDG creates three additional edges to handle function calls: (1) call edge, (2) parameter-in edge, and
(3) parameter-out edge. A call edge connects the node at the call site to the entry node of the called
procedure. Parameter-in edges connect the actual-in parameter nodes to the formal-in parameter nodes of
the called function, and parameter-out edges connect the formal-out nodes to the actual-out nodes.
Fig.~\ref{fig:sdg} shows an SDG for two functions, $f_1$ and $f_2$, where $f_1$ calls $f_2$.
When $f_1$ calls $f_2$ during the program flow, a call edge from the call site in caller $f_1$ to the
entry node of callee $f_2$ represents this calling relationship. Also, the arguments passed by the
caller are represented by the \textit{actual\_in} nodes, and the \textit{formal\_in} nodes represent the
arguments received by the callee. The returned value from the caller is represented
by the \textit{formal\_out} node, whereas the value received by the callee represents the \textit{actual\_out} 
node. As shown in Fig.~\ref{fig:sdg}, the solid and dotted lines represent the control and data dependencies 
between the SDG nodes, respectively.

\subsection{Sequence Models}
Sequence models are ML-based models that can analyze data with sequential dependencies. Time-series 
data, video and audio clips, and text streams are a few examples of sequential data. %A popular deep learning model used for sequential modeling is the recurrent neural network (RNN). Unlike traditional %neural networks, RNNs can remember their previous inputs, which they consider during inference. As shown in Fig. \ref{fig:rnn}, the RNN architecture can be unfolded and represented as a chain of neural networks sharing the weights over time instances. An RNN cell propagates a hidden state $h_t$ to the next RNN cell. The hidden state $h_t$ encodes the entire history of the sequence so far in a fixed-length vector. Although RNNs perform well on some tasks, they cannot process long-range dependencies. They require deep neural networks to do so. While training deep networks, gradients (or error derivatives) decay exponentially. This decay leads to the vanishing gradient problem. Due to degraded gradients, weights in the deep layers of the neural network are not trained sufficiently. This limitation prevents RNNs from analyzing long-range dependencies.

\begin{comment}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.34]{images/RNN.pdf}
    \caption{The RNN architecture: $x_t$, $h_t$, and $y_t$ represent the input, hidden state, and
output at time $t$, respectively.}
    \label{fig:rnn}
\end{figure}

\end{comment}


\subsubsection{LSTM}

%Hochreiter et al.~\cite{hochreiter1997long} proposed LSTMs to overcome the vanishing gradient problem. 
A popular deep learning model used for sequential modeling is the LSTM. This is because LSTMs are capable of handling long-range sequential dependencies. %LSTMs forward the hidden state $h_t$ and the cell state $c_t$ to the next LSTM cell. 
%As shown in Fig.~\ref{fig:lstm-cell}, 
LSTM cells have three unique gates: forget, input, and output. 
%LSTMs use these gates to control gradient propagation in the network. 
The gates help the network manipulate memory by omitting unimportant information while retaining helpful information. 
%LSTMs are used in many practical applications, including Apple's Siri and Google's voice search. However, LSTMs have their limitations. 
The LSTM cells compress the entire sequence history into the hidden state, which is a fixed-length vector. This compression limits the LSTM's performance in capturing semantic relationships between elements spread far apart in long sequences. 

\begin{comment}

\begin{figure}[h]

\vspace{-0.5cm}

\centering
\includegraphics[width=1.03\linewidth,scale=1.2, height =0.6\linewidth]{images/LSTM.pdf}
\vspace*{-4mm}
\caption{The architecture of an LSTM cell~\cite{jenkins-lstm}} 

\label{fig:lstm-cell}
%\vspace{-0.1cm}
\end{figure}

\end{comment}

Security analysts often use LSTMs and their variants to analyze system-call sequences for vulnerability detection. 
More sophisticated versions of the LSTM, like bidirectional-LSTMs \cite{li2018vuldeepecker} and 
CNN-LSTMs \cite{8322752}, usually achieve good performance over vanilla LSTM models. However, they require 
significant computation overheads due to their increased complexities. Therefore, we compare ML-FEED with the state-of-the-art lightweight LSTM model with reasonable accuracy while taking minimal computation time. As shown in Fig.~\ref{fig:lstm-architecture}, this architecture is a cascade of an LSTM cell followed by a feedforward neural network. 

\begin{figure}[h]
\centering
%\vspace{-0.7cm}
\includegraphics[width=1.05\linewidth,scale=1.2, height =0.66\linewidth]{images/LSTM-architecture.pdf}
\caption{The high-level LSTM-based architecture for vulnerability exploit detection. $x_t$, $h_t$, $c_t$, and $y_t$ denote the input feature vector, hidden state, cell state, and multi-label output at time $t$, respectively.} 
\label{fig:lstm-architecture}
%\vspace{-0.2cm}
\end{figure}

We train the LSTM model on sequences of feature vectors and their corresponding labels. Unlike most prior research, 
we do not wait to complete program execution to begin inference. Instead, we train the LSTM model to predict the 
occurrence of an exploit after every API call. Such an inference at every time step enables us to detect exploits 
efficiently and halt program execution when an exploit is detected. During inference, first, we convert the API calls into feature vectors based on the method described in Section \ref{sec:Feature_engineering}. 
Then, the LSTM cell receives the feature vector of the API call and outputs a cell state and a hidden state. The 
hidden state encapsulates the sequence history encountered so far. The cell state is represented by an $n$-dimensional binary output vector where $n$ is the number of exploit categories in our threat model. The cell state indicates the exploits the API call has triggered. If the 
current API call does not trigger any exploit, the cell state is a zero vector. When the following API call executes, the LSTM analyzes the features of the new API call along with the current hidden state. As a 
result, it outputs an updated hidden state and cell state. This process continues till the end of program 
execution.



\subsubsection{Transformer}
Transformers are another category of sequence analysis models~\cite{wu2021literature}. Recently, transformers have become popular because they are more successful at capturing long-range dependencies with the help of the attention mechanism. This mechanism 
considers the entire series during inference and decides which parts to focus on at the current 
time instance. Transformers use multiple attention mechanisms to compute a context vector. This vector determines how to prioritize the different elements of a sequence. 
Transformers use multiple attention modules to attain extraordinary discriminative power. This mechanism 
is known as multi-head attention. It has played a vital role in the success of transformer 
models.

Furthermore, their advanced semantic 
knowledge representation enables sophisticated modeling of semantically-similar functions. Although very
successful, transformers are often huge models that incur enormous computation overheads. Transformer architectures 
that have performed well on NLP tasks have also been successful in system-call sequence analysis. Some of the most  
popular transformer architectures used for detecting vulnerabilities include the generative pre-trained
(GPT) transformer and its variants~\cite{radford2019language}, BERT~\cite{devlin2018bert} and BART~\cite{lewis2019bart}. The GPT family of transformers is a decoder-based model, 
whereas the BERT and BART transformers are encoder-based models. We experiment with the GPT-2 transformer because 
it is easier to model our problem statement with a decoder model.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth,scale=0.8, height =0.6\linewidth]{images/GPT-2.pdf}
\caption{A high-level overview of the GPT-2 architecture} 
\label{fig:GPT-2}
\vspace{1mm}
\end{figure}

The GPT-2 transformer is a current state-of-the-art open-source transformer model for NLP tasks. It is an advanced version of the GPT transformer that takes a partial sentence as input and successfully predicts the next 
word. It foretells the next word by computing the output probability of all the words in its vocabulary. In our 
case, instead of calculating the output probability of words, the model calculates the output probability of the 
API call triggering any exploit in our threat model.

We show the GPT-2 architecture in Fig.~\ref{fig:GPT-2}. It uses word embeddings and positional embeddings. 
Word embeddings successfully capture the semantic closeness of the words in the vocabulary, whereas positional 
embeddings enable an understanding of the context. %Word embeddings of API names are present in our feature vectors as well. 

The masked self-attention layers of the GPT transformers make them unique. They inform the transformer 
which subsequence to focus on while making decisions. We carefully design our masks and labels to train the model 
on subsequences of the same exploit chain during training. We use the most lightweight of the four open-source 
GPT-2 models. Even the smallest GPT-2 model has 117 million parameters, which is much larger than the 46,788 
parameters used in the ML-FEED model. %Our GPT-2 model has 12 decoder layers with 12 attention heads in each self-attention layer. 
Another drawback of transformers is that they cannot process sequences of all lengths. The 
GPT-2 model can process a series of a maximum of 1024 API calls.



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
This section discusses the limitations of ML-FEED. It also proposes potential future work that may address some of these limitations. 

First, ML-FEED cannot detect vulnerabilities that require dynamic program analysis. In ML-FEED, we train our model with instructions 
statically generated from the source code. While this method efficiently detects potential program paths that 
can be exploited during execution, its efficiency does not transfer to vulnerabilities that require dynamic 
program analysis. For example, let us consider the following statement: \textit{``byte foo = (byte)(bar + 1)''}. 
Our model can efficiently detect whether variable $bar$ may flow into a vulnerable sink during program execution 
without reasoning about the variable's actual value. However, if variable $bar$ contains a user-controlled input, 
this statement can cause \textit{integer overflow} (if \textit{bar == Byte.MAX\_VALUE}). As we do not reason about 
the values of expressions or values that a variable may hold at run-time, such vulnerabilities are out of the 
scope of this work. Combining static and dynamic program traces will enable our model to capture such 
vulnerabilities, which we leave as future work.

Finally, because ML-FEED analyzes the source codes, it has access to the names of the functions and APIs called during execution. However, these names may be deleted (or stripped) in executable binaries of applications to reduce the size of the deployed code. We plan to extend our analysis to such stripped binaries in future work. We need to identify the function names from the program structure in the binaries to do this. Recent research proposes multiple ML-based approaches to successfully do this~\cite{patrick2020probabilistic}. A potential approach to address this research problem is to first predict the function names in the executable binaries using ML. Then, we can input these name predictions into ML-FEED.

Third, we can combine our methodology with automatic extraction of vulnerability fingerprints from the CWE database in future research. This will reduce human intervention in the process. We currently use the CWE database to manually define the vulnerability fingerprint at a high level, which allows us to (automatically) extract a large number of queries based on the CVE database.

Fourth, we use SDG to extract the vulnerable API sequences from the programs in our dataset. However, there are many other graph representations, such as PDG, CPG, etc., that have been proven to be effective for vulnerability detection. Since we train our model using the sequences extracted from the graph, it can be easily extended for other graph representations.

Finally, this article strives to balance identifying unknown vulnerabilities and increasing the efficiency of detecting known vulnerabilities. During our experiments, we discovered a trade-off between the efficiency and efficacy of ML-based vulnerability classifiers. Sophisticated and massive models like transformers may process the intricate semantics of convoluted attack sequences of \textit{zero-day} exploits better than our model for some CWEs. However, our model is designed to learn the behavior of \textit{known} vulnerabilities to identify them more efficiently than previous methods. Thus, it is challenging for ML-FEED to detect zero-day exploits in the wild. In the future, we plan to infer new vulnerability fingerprints from known fingerprints, enabling us to better identify new vulnerabilities. In addition, while our goal is to detect vulnerable program flows, our proposed method does not prevent the execution of vulnerable programs. We plan to explore how ML-FEED can be incorporated with existing defense mechanisms, such as control flow integrity-based approaches~\cite{hu2018enforcing}, to accomplish this.


==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> threat_model.tex <==
\section{Threat Model}~\label{sec:threat}
We intend to detect vulnerability exploits by classifying control and data flow transfers over an 
application run. Thus, we target attacks that modify control flow, data flow, and data invariants during the execution of benign applications. Our threat model covers many vulnerabilities, such as SQL injection, remote 
code execution, cross-site scripting, and unsafe storage of passwords. These vulnerabilities frequently 
occur in both web and native applications. We assume that the applications (e.g., source code, binaries) work as an honest host for their internal resources (e.g., database). However, we assume that the attackers can control internal resources or the application execution flow by exploiting user-controlled inputs or external services (e.g., remote API calls).

\begin{comment}

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.5]{images/clasted-overview.pdf}
    \caption{Overview of ML-FEED}
    \label{fig:overview}
    \vspace{0.5cm}
\end{figure*}

\end{comment}


